Personalized Benchmarking with the Ludwig Benchmarking Toolkit

The rapid proliferation of machine learning models across domains and deployment settings has given rise to various communities (e.g. industry practitioners) which seek to benchmark models across tasks and objectives of personal value. Unfortunately, these users cannot use standard benchmark results to perform such value-driven comparisons as traditional benchmarks evaluate models on a single objective (e.g. average accuracy) and fail to facilitate a standardized training framework that controls for confounding variables (e.g. computational budget), making fair comparisons difficult. To address these challenges, we introduce the open-source Ludwig Benchmarking Toolkit (LBT), a personalized benchmarking toolkit for running end-to-end benchmark studies (from hyperparameter optimization to evaluation) across an easily extensible set of tasks, deep learning models, datasets and evaluation metrics. LBT provides a configurable interface for controlling training and customizing evaluation, a standardized training framework for eliminating confounding variables, and support for multi-objective evaluation. We demonstrate how LBT can be used to create personalized benchmark studies with a large-scale comparative analysis for text classification across 7 models and 9 datasets. We explore the trade-offs between inference latency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness, showing how LBT can be used to satisfy various benchmarking objectives.

==> src/abstract_old.tex <==
\begin{abstract}
 In the machine learning (ML) community, There is a need for personalized model benchmarking which allows researchers and practitioners to compare models on the tasks and evaluation criteria they care about. 
%
Standard benchmarking practices fall short in enabling user-specific benchmark studies as they typically evaluate models on a single, domain-agnostic objective (e.g. accuracy), exclude practically useful information (e.g. training speed), and don't provide a standardized training framework that controls for confounding variables (e.g. computational budget) that makes fair comparisons possible. 
%
% To address these challenges, we introduce the new open-source Ludwig Benchmarking Toolkit (LBT), a personalized benchmarking toolkit for running end-to-end benchmark studies across an easily extensible set of tasks, deep learning models, standard datasets and evaluation metrics.
To address these challenges, we introduce and open-source the Ludwig Benchmarking Toolkit (LBT), a personalized benchmarking toolkit for running end-to-end benchmark studies across an easily extensible set of tasks, deep learning models, standard datasets and evaluation metrics.
%
LBT enables researchers and industry practitioners to build user-specific benchmark studies and perform rich, comparative model meta-analyses by providing a standardized training framework for controlling confounding variables (e.g., hyperparameter tuning budget, preprocessing methods) and by supporting multi-objective evaluation. 
%
We demonstrate the efficacy of LBT with a large-scale comparative analysis for text classification across 7 models and 9 datasets. Our results show how LBT can be helpful in identify tradeoffs between inference efficiency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness.

%LBT enables users to build user-specific benchmark studies and perform rich, comparative model meta-analyses by providing(i) a configuration-driven process to construct benchmark studies by defining datasets, tasks, performance criteria, models and hyperparameter settings, that can be easily extended to support more of each, (ii) a standardized training framework that controls for confounding variables such as hyperparameter tuning budget, preprocessing methods, and differences in training procedures and parameters and (iii) multi-objective evaluation that measures several standard metrics, cost, efficiency, robustness and sub-population based performance. We demonstrate the efficacy of LBT with a large-scale comparative analysis for text classification across 7 models and 9 datasets. Our results show how LBT helps identify tradeoffs between inference efficiency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness.
\end{abstract}


%Benchmarking is a standard practice for comparing machine learning models and has helped drive advances across tasks and modalities. % [original] Traditional, leaderboard-style benchmarks evaluate models on a single objective (e.g. accuracy), exclude practically useful information (e.g. inference latency) and fail to control for confounding variables (e.g. computational budget). %[possible alternative - Avanika] %[Piero]: Traditional, leaderboard-style benchmarks do not provide a standardize implementation, which leads to evaluating models on a single objective (e.g. accuracy), exclude practically useful information (e.g. inference latency) and not controlling for confounding variables (e.g. computational budget). Traditional, leaderboard-style benchmarks evaluate models on a single objective (e.g. accuracy), exclude practically useful information (e.g. inference latency), and don't provide a standardized training framework that controls for confounding variables (e.g. computational budget).To address these challenges, we introduce the new open-source Ludwig Benchmarking Toolkit (LBT), a framework for building standardized, multi-objective, and extensible model benchmarking studies.%LBT supports classification, regression and generation tasks across multiple modalities, datasets and deep-learning models off-the-shelf, it only requires users to declare the datasets, tasks, performance criteria, models and hyperaparameter sets to use for building a benchmark, and can be easily be extended to support more of each. LBT enables users to perform rich, comparative model meta-analyses by providing(i) a configuration-driven process to construct benchmark studies by defining datasets, tasks, performance criteria, models and hyperparameter settings, and can be easily extended to support more of each (ii) a standardized training framework that controls for confounding variables such as hyperparameter tuning budget, preprocessing methods, and differences in training procedures and parameters, (iii) multi-objective evaluation that measures several standard metrics, cost, efficiency, robustness and sub-population based performance, and  (iv) access to a collaborative hub for sharing and extending experiments. We demonstrate the efficacy of LBT with a large-scale comparative analysis for text classification across 7 models and 9 datasets. Our results show how LBT helps identifying tradeoffs between inference efficiency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness.
%

%%% Updated abstract ends here

%%% Old abstract

% Leaderboard-style benchmarking is the standard practice for comparing models in the machine learning community and has helped drive advances across many tasks. Ideally, benchmarking should provide clarity on the effect that model architecture differences have on task performance and enable for accurate model comparisons on the basis of multiple objectives (e.g., efficiency, robustness, accuracy). Unfortunately, the conventional practices fall short of giving practitioners and researchers the ability to identify the best models for the tasks and criteria they care about, since they evaluate models based on a single objective (i.e., accuracy), fail to report statistics of practical concern like model size and inference latency and do not control for confounding variables such as computation budget or choice of optimizer that make fair model comparisons infeasible.To address these issues, we present a novel conceptualization of model benchmarking via the open-source Ludwig Benchmarking Toolkit (LBT): an end-to-end framework for conducting standardized, extensible, and multi-objective benchmark studies. The toolkit supports classification, regression and gerneration tasks across multiple modalities and includes a wide and extensible set of ready-to-use datasets and deep learning models. LBT enables researchers and practitioners to accurately compare deep-learning models and perform rich, meta-analyses by (i) providing a standardized training framework in which users can easily control for confounding variables, (ii) enabling multi-objective evaluation by reporting metrics and providing tooling that measure cost and efficiency, robustness and sub-population based performance, and (iii) facilitating access to a collaborative hub for sharing and extending benchmark experiments. We demonstrate the efficacy of LBT by running a large-scale comparative analysis for text classification across 7 models on 9 datasets. To our knowledge, LBT is the only toolkit for running end-to-end, multi-objective benchmark studies of deep learning models. 

%%% Old abstract ends here


==> src/checklist.tex <==
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{discussion_and_conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{sec:additional_casestudy_details}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{case_study} and ~\ref{appendix:metrics}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{case_study}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you citep the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See page 1 for link to LBT code repository} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> src/introduction_old.tex <==
\section{Introduction}

Benchmarking has emerged as an important practice to measure progress in machine learning. % and clarifying the advantages and limitations of techniques. 
%
Typically, benchmarking is done through leaderboards, where the participant's objective is to maximize a performance criterion on a challenging task or dataset.
%
% Here, the benchmark designers are responsible for formulating a challenging task, collecting and preparing data, selecting the performance criterion, preparing a submission protocol, and eventually hosting the leaderboard where submitted results are ranked.
%
Prominent examples of these benchmarks include GLUE~\citep{wang2019glue}, SuperGLUE~\citep{wang2020superglue} and SQuAD~\citep{rajpurkar2016squad}, among many others. 

As deep learning models become increasingly proficient at maximizing performance criteria like accuracy and F1 scores, attention and urgency has shifted towards the need for more personalized, thorough and thoughtful benchmarking. %, rather than a ``winner-takes-all" approach. 
%
Several challenges to this ``winner-takes-all" style of benchmarking have emerged. 


First, recent work has highlighted the need for personalized benchmarks that better cater to an individual practitioner's needs \citep{ethayarajh2020utility}.
%
Existing benchmarks provide little utility to an individual who wants to compare a collection of models on multiple objectives such as robustness, efficiency, fairness, carbon footprint or other properties---all aspects that are highly valued by researchers and practitioners~\citep{ethayarajh2020utility, linzen-2020-accelerate}.
%
Instead, leaderboards have excelled at catalyzing the larger research community to make progress on a task e.g. moving from xx\% to yy\% on GLUE in under 2 years with the emergence of transformers~\cite{}. 
%


Second, a general goal for benchmarking is to aid researchers in teasing apart exactly \emph{why} some models perform better or worse. 
%
The mechanism adopted by leaderboard benchmarks precludes the ability to precisely answer such questions
%
%The self-reporting mechanism adopted by leaderboard benchmarks precludes the ability to precisely answer questions about \emph{why} models are better or worse.
%
%This is simply
because submitted models vary substantially: in the data, compute resources and preprocessing they use \citep{Rogers_2019_leaderboards}, and in their implementation of the model architecture, training protocol and hyperparameter tuning. %, and in the hardware and infrastructure they use to train.
%
These confounding factors make it difficult to draw any conclusion about what parts of an implementation are ultimately responsible for its performance, especially since these factors may matter even more than architecture differences~\citep{sun2018models, schmidt2021descending, kandasamy2020tuning, abenmacher2020comparability}. 
%
% Ideally, It is precisely these confounding factors that researchers aim to disentangle in order to advance our understanding 

Lastly, the shift towards personalized benchmarks changes the nature of the burden on benchmark designers, from dataset collection and curation, to careful evaluation and implementation.
%
The major burden so far has been in formulating a challenging task, collecting and preparing data, and selecting an appropriate performance criterion to capture progress on the task. 
%
Progress in benchmarking has largely focused on making it easier to address benchmark stagnation, by injecting mechanisms for data collection that evolve a benchmark over time~\cite{nie2020adversarial}.
% 
However, the shift to personalization necessitates the development of new tools that make it easier to create personalized benchmarking studies.

In summary, these challenges highlight the need for personalized benchmarking tools that complement existing leaderboard-style benchmarks, and let researchers, practitioners and domain experts (i) perform multi-objective evaluation, (ii) control for confounding variables, and (iii) extend and customize evaluation and training.


% Taken together, these challenges point to the need for new tools that support researchers and practitioners as they move towards the personalized benchmarking.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD INTRO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% With the rapid proliferation of new tasks and model architectures, there is increasing interest amongst researchers to compare models in a more accurate and robust manner \cite{ethayarajh2020utility,liu2021explainaboard}, to understand the relationships between models, tasks, and datasets \cite{ezencan2020comparison}, and to study the tradeoffs between fine-grained model performance and other criteria beyond accuracy such as efficiency, cost, and robustness \cite{jacobsen2021optimal, schwartz2019green, strubell2019energy}. 
%
% Well-defined systems for standardized and transparent model benchmarking can help the community in the aforementioned pursuits.


% \noindent In the machine learning community, leaderboard-style benchmarks represent the standard procedure for benchmarking, wherein researchers presenting a new approach or architecture validate their work on an established set of datasets for a given task. 
%
% There are two primary issues with this standard practice that make robust and accurate model benchmarking difficult and that we seek to address in our work.


% \noindent Firstly, there are several confounding factors that may make understanding the realized benefits of a newly proposed architecture unclear. 
%
% While most canonical benchmarks like GLUE \cite{wang2018glue}, SQuAD \cite{rajpurkar2018know}, and ImageNet \cite{russakovsky2015imagenet} provide a standard evaluation set-up (via datasets and a static evaluation metric) they do not control for confounding variables such as training time, the number of hyperparameters tested, and training parameters such as the type of optimizer or learning rate schedule, that can all impact the performance of the final model, potentially even more than differences in the model architecture \cite{sun2018models, schmidt2021descending, kandasamy2020tuning, abenmacher2020comparability}. 
%
% Due to this lack of standardization, it is difficult to draw conclusions about the correlation between architectures and performance on the basis of self-reported results alone.

% \noindent Secondly, 
% %there is a general lack of rigor when reporting experimental results and it is uncommon for researchers to publish statistics of practical concern such as efficiency, latency, model size, and training time when introducing new contributions. Moreover, 
% the majority of existing reported results and benchmarks focus on performance-based evaluation and report a single evaluation metric,  and lack aspects of practical concern such as efficiency, latency, cost, model size,  training time, fairness, and robustness which are highly valued amongst the researchers and practitioners \cite{ethayarajh2020utility, linzen-2020-accelerate}.  Thus, using these results to perform multi-objective comparisons and to empirically study performance tradeoffs is difficult, if not impossible. Given that there exists a wide range of stakeholders seeking to perform benchmarking analysis spanning from ML researchers, software engineers, to social scientists, enabling multi-objective comparisons is of utmost value. 

% \noindent As such, there exists a need for a new system for model benchmarking that lets researchers and practioners accurately compare and thoroughly benchmark models by (i) providing a standardized training framework in which users can easily control for confounding variables, (ii) collecting a wide range of metrics beyond accuracy to perform multi-objective evaluation, and (iii) making it easy to share and extend benchmark studies for future benchmarking research or other empirical studies.

% \subsection{Contribution}

We take a first step in this direction and introduce the {\bf Ludwig Benchmarking Toolkit (LBT)}, a personalized benchmarking toolkit that allows users to setup and run \textit{multi-objective, standardized and extensible} benchmarking studies with ease. 
% 
In particular, LBT has the following properties:

%In a typical benchmark study in LBT, a user will choose a task(s), a set of models to compare, and several datasets for evaluation. We describe the key attributes of the system below:

\begin{enumerate}[leftmargin=*]
\item \textbf{Multi-objective.} 
To provide greater support for the various evaluation metrics a personalized benchmark might require, LBT expands the set of evaluation criteria beyond standard performance-based evaluation (e.g. accuracy and F1) to include cost, size, training speed, inference efficiency and carbon footprint. Furthermore, it includes integrations with two popular open-source evaluation toolkits (\cite{goel2021robustness}, \cite{morris2020textattack}) which allows comparing model robustness and slice/sub-population based performance.
%
% Users can introduce new evaluation metrics to further customizing their evaluation criteria to their own needs. 
%

%Access to this broad set of evaluation criteria and tooling researchers to perform rich meta analyses as part of their experiments and understand model performance in a more fine-grained manner.

\item \textbf{Standardized.} To enable for fair comparisons of models trained using the toolkit, LBT implements a standardized training framework that ensures that every model can be trained using the same dataset splits, preprocessing techniques, training loop, learning rate scheduler, and hyperparameter ranges and sampling budget if required. 
%
This framework is exposed via a configuration-file interface wherein users running an experiment specify a set of models, datasets, and tasks, define the hyperparameter search space for optimization and set training parameters (e.g. learning rate). When configuring the hyperparameter search space and training settings, users choose which variables to hold constant across models such as training time, the choice of optimizer, preprocessing techniques, and the hyperparameter tuning budget, controlling for any potential confounds.
 %
Built on top of the Ludwig Deep Learning Package (Ludwig) ~\cite{molino2019ludwig}, LBT provides out-of-the-box support for training cutting-edge deep learning models that span classification, regression and generation tasks across multiple modalities. 

\item \textbf{Extensible.} 
To further support the creation of more personalized benchmark studies, LBT is designed such that it is simple to extend the scope of supported models, datasets and metrics within the toolkit.
%
Specifically, LBT provides users with explicit mechanisms for introducing custom datasets, metrics, and models.
%
Moreover, expanding the breadth of completed experiments (by adding more datasets, models and evaluation metrics) is simple. Setting up benchmarking experiments requires populating a handful of configuration files and expanding them only requires adding entries in those files (e.g. an additional dataset in the datasets configuration file).
%These configuration files provide a snapshot of all experimental settings used in the original experiment. Thus, with access to these configuration files, extending the scope of an experiment is trivial.
%

 

%Thus, we hope that our benchmarking toolkit and research hub will serve as a collaborative place where researchers can crowdsource benchmark experiments and build upon existing studies. %We envision these benchmark studies to be viewed as living, breathing leaderboards that communities can coalesce around and grow over time as new models, datasets, and evaluation criteria are introduced. 
    
\end{enumerate}
%
We propose that LBT is useful to researchers, industry practioners and domain experts for creating personalized benchmarking studies.
%
We demonstrate how researchers and industry practioners might conduct a personalized benchmark study through a {\bf large-scale, multi-objective benchmarking analysis} of $7$ deep learning models across a diverse set of $9$ text classification datasets.
%
In our analysis, we empirically test a number of hypothesis of relevance to both researchers and industry practioners such as the tradeoffs between inference efficiency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness, all while controlling for important confounding factors.
%
Our results show that, of the models we compared, DistilBERT has the best inference efficiency and performance trade-off, BERT is the least robust to adversarial attacks and pre-trained models do not always converge faster than models trained from scratch.


% Using LBT, we empirically test hypotheses regarding the tradeoffs between inference efficiency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness, all while controlling for important confounding factors. 

%Our results show that, of the models we compared, DistilBERT has the best inference efficiency and performance trade-off, BERT is the least robust to adversarial attacks and pre-trained models do not always converge faster than models trained from scratch.

\begin{figure}
    \centering
        \captionsetup{justification=centering}
        \includegraphics[width=1\textwidth]{images/toolkit-diagram.pdf}
    \caption{LBT Toolkit Overview}
\end{figure}

% To address the aforementioned problems, a new open-source toolkit for creating robust and extensible, multi-objective benchmark studies.
% We outline our key contributions as follows:

% \textbf{1. Ludwig Benchmarking Toolkit (LBT)}, a framework for running standardized, extensible and multi-objective benchmarking experiments. \an{Modify the above to be more explicit about what LBT is, assuming that we have concerns about lack of clarity} Built on top of the Ludwig Deep Learning Package [cite], LBT provides support for benchmarking models on classification, regression and generation tasks across multiple modalities. The toolkit contains  out-of-the-box support for several cutting-edge deep learning models and standard datasets and supports integrating additional models and datasets. In a typical benchmark study in LBT, a user will choose a task(s), a set of models to compare, and several datasets for evaluation. We describe the key attributes of the system below:

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Standardized}: LBT provides a standardized training framework
%     %that is non-existent in protoypical benchmarking practices. The framework contains a declarative interface for specifying variables that are to be held constant across all models, thus eliminating any possible confounds and ensuring fair model comparisons.
%     that ensures that every model is trained using the same preprocessing, training loop, learning rate scheduler, splits, hyperparameter ranges and number of hyperparameters samples. This eliminates confounds and allow for fair model comparisons.
%     \item \textbf{Extensible}: The configuration file driven design of the benchmarking framework makes it easy to reproduce experiments (see \hyperlink{section.2}{Section 2}). In addition to reproducibility, it is simple to extend the scope of an existing study by adding more datasets, models, and metrics. Thus, we hope that our benchmarking toolkit and research hub will serve as a collaborative place where researchers can crowdsource benchmark experiments and build upon existing studies. We envision these benchmark studies to be viewed as living, breathing leaderboards that communities can coalesce around and grow over time as new models, datasets, and evaluation criteria are introduced. 
%     \item  \textbf{Multi-objective evaluation}: Unlike most existing benchmarks which solely rely on performance-based evaluation (e.g., maximizing accuracy or F1 score), LBT expands the set of evaluation criteria to include cost, size, efficiency, robustness and slice/sub-population based performance. Moreover, users can introduce new evaluation metrics, further customizing their evaluation criteria to their own needs. Access to this expansive set of evaluation criteria and tooling will enable researchers to perform rich meta analyses as part of their experiments and understand model performance in a more fine-grained manner.
% \end{itemize}

% \textbf{2. Large scale comparative analysis for text classification}. Using LBT, we perform a large-scale benchmarking analysis of 7 cutting-edge deep learning NLP models across a large and diverse set of text classification datasets. With this study, we demonstrate the utility of LBT in enabling standardized, multi-objective benchmark studies and empirically test hypotheses regarding the tradeoffs between inference efficiency and performance, relationships between dataset attributes and performance, and the effects of pretraining on convergence and robustness. 
   


==> src/persona.tex <==


\subsection{Benchmarking for Value-Driven Communities}
We start by describing the users that LBT primarily targets. We consider user communities whose utility is aligned with understanding and advancing objectives beyond average performance. In particular, we are interested in communities that satisfy the following characteristics:

\begin{itemize}
    \item {\bf Value driven.} The community is aligned by a set of values for which average accuracy is not a good proxy. Users' goals are primarily to compare models with respect to one or more objectives beyond average performance. 
    \item {\bf Require standardization.} Users place strong emphasis on conducting clear, standardized analyses, in order to advance understanding and draw accurate conclusions.
    \item {\bf Prefer automation.} Users value the ability to control and configure their benchmarks, but would prefer or be willing to write as little code as possible. 
\end{itemize}

Taken together, these characteristics allow us to describe and target communities that \citep{ethayarajh2020utility} argue remain underserved by traditional benchmarks. 
%
To ground this discussion, we provide examples of $3$ subcommunities of ML research, industry practitioners and consumers of machine learning.
\begin{itemize}
    \item {\bf ML researchers interested in performing comparative meta-analyses.}
    
    \item {\bf Industry practitioners interested in deployment-readiness.} 
    
    \item {\bf Subject-matter experts interested in task-specific performance.}
    
\end{itemize}


